Gaussian Robust Classification

Supervised learning is all about the ability to generalize knowledge. Specifically, the goal of the learning is to train a classifier using training data, in such a way that it will be capable of classifying new unseen data correctly. In order to acheive this goal, it is important to carefully design the learner, so it will not overfit the training data. The later can is done usually by adding a regularization term. The statistical learning theory explains the success of this method by claiming that it restricts the complexity of the learned model. This explanation, however, is rather abstract and does not have a geometric intuition. The generalization error of a classifier may be thought of as correlated with its robustness to perturbations of the data: a classifier that copes with disturbance is expected to generalize well. Indeed, Xu et al. [2009] have shown that the SVM formulation is equivalent to a robust optimization (RO) formulation, in which an adversary displaces the training and testing points within a ball of pre-determined radius. In this work we explore a different kind of robustness, namely changing each data point with a Gaussian cloud centered at the sample. Loss is evaluated as the expectation of an underlying loss function on the cloud. This setup fits the fact that in many applications, the data is sampled along with noise. We develop an RO framework, in which the adversary chooses the covariance of the noise. In our algorithm named GURU, the tuning parameter is a spectral bound on the noise, thus it can be estimated using physical or applicative considerations. Our experiments show that this framework performs as well as SVM and even slightly better in some cases. Generalizations for Mercer kernels and for the multiclass case are presented as well. We also show that our framework may be further generalized, using the technique of convex perspective functions.

==> Motivation.tex <==
\section{Motivation}

The fundamental task of supervised learning is classifying new data, based on understanding gained on a training set. This property is commonly referred to as Generalization, i.e. the ability to have a low error rate on the test set.
In the traditional supervised learning setting, one tries to minimize the expected risk of the zero-one loss over the distribution of the data. In most of the cases, however, this distribution is unknow. A walk-around this problem is the technique of empirical risk minimization (ERM), i.e. optimizing the performance over the training set. Two major problems arise in this case. First, there may be multiple classifiers that perform the same on the training data, and one should apply a criterion to choose among them. Second, minimizing the loss over the training set solely will most likely result in overfitting. The PAC theory analyzes the difference between the actual and the empirical risks and tries to bound it. Multiple threads of reasoning acount for the incorporation of an additive regularization term to the objective of the optimization problem: Occam's razor, maximal margin (see above), etc. \newline
It has been shown by Xu et al (Shie Mannor's paper) that ...
This method can be shown to be optimal in the case that no other information is available (ref). In many real world applications, however, the data we are given is corrupted by noise. Taking this noise into consideration is thus only sensible in order to minimize the actual risk. \newline
Previous works that have incorporated a noise model into the learning setup (TSVC of Zhang) tried to learn a better classifier by presenting the learning algorithm 'more reasonable' samples. Our approach, however, is that the noise is inherent to the process, thus we must learn how to classify when it is present. To that extent, we introduce an adversarial model, in which our goal is to minimize the worst case loss:
\be
\min_{\ww} \sum_m \max_{\theta\in S}\int p(\hat\xx;\xx^m,\theta) \left[ 1-y^m\hat\xx\cdot \ww \right]_{+} d\hat\xx  
\ee
where $p(\cdot;\xx^m,\theta)$ is a noise model, having its mean at $\xx^m$ and its parameter $\theta$ taken out of the constrained set $S$, that will be discussed later. In many cases it is hard to give an exact and tractable algorithm for this setup (I think that either zhang or the idiap report claimed that it is not possible even in the gaussian casem but I am not sure..). In this work we show that in a bunch of simple yet usefull cases (gaussian and laplacian, any more?) it may be done. As we show in the subsequent sections, classifiers leanrt using this setup are notably more robust, to the extent of having better generalization performance than standard SVMs (TSVs? others?). \newline
The rest of the paper is organized as follows...


==> OurContrib.tex <==
\section{Our Contribution}

In this work we present a new robust-learning setup and show that it yields a learning algorithm which generalizes as good as SVM. By learning a classifier which is robust to the worst case Gaussian disturbance, we derive a novel family of smooth loss functions. We show that these functions contain a multiplicative norm term (that might be though of as linear term by taking the logarithm).
\newline
We devise an SGD based algorithm to solve for the optimal classifier in our setup, both in the binary and in the multiclass case. At last, we show that our algorithm may be generalized to Mercer kernels, using our obseravtion that the norm of the classifier may be updated on-the-fly which low computational costs.


==> SVM.tex <==
\section{Support Vector Machines}
sad


==> badDual.tex <==
\subsubsection{Unsuccessfull Approach}
I have played around this dual issue for long time. my obeservation is that if we try to derive the dual of the problem without the explicit regularization after substituting the optimal $\Sigma$ we get inreasonable dual (very similar to what we have discussed in the cofee shop): Let us try to derive the dual of the above problem
\be
\min_{\ww} \sum_m {1\over{\sqrt{2\pi\beta}}}\int e^{-{u^2\over 2\beta}}\left[ 1-y^m \ww\cdot\xx^m+u \right]_{+} du
\ee
Introducing slacks we get
\be
\min_{\ww,\xi^1(u),\xi^2(u),...,\xi^N(u)} \sum_m {1\over{\sqrt{2\pi\beta}}}\int e^{-{u^2\over 2\beta}}\xi^m(u) du  
\ee
\begin{align}
\text{s.t. } \forall i\forall u\quad & \xi^i(u)\geq 0 \nonumber \\
&\xi^i(u)-1+y^i \ww\cdot\xx^i-u\geq 0
\end{align}
The lagrangian is thus
\begin{align}
\mathcal{L}\left(\ww,\xi^i(u),\lambda_i(u),\delta_i(u)\right)=&\sum_m {1\over\sqrt{2\pi\beta}}\int e^{-{u^2\over 2\beta}}\xi^m(u) du \nonumber \\ -&\sum_m{\int{\lambda^m(u)\left( {\xi^m(u)-1+y^m \ww\cdot\xx^m-u}\right)} du} \nonumber \\ - &\sum_m {\int\delta^m(u)\xi^m(u) du}
\end{align}
The next step would be to find extremum w.r.t the primals. To that end let us calculate the following derivatives:
\be
\label{eq:firstCond}
{\partial\mathcal{L}\over\partial\ww}=  - \sum_m {y^m\xx^m\int\lambda^m(u) du}
\ee
\be
{\partial\mathcal{L}\over\partial\xi^i(u)}={1\over\sqrt{2\pi\beta}}e^{-{u^2\over 2\beta}}-\lambda^i(u)-\delta^i(u)
\ee
Multiplying \eqref{eq:firstCond} by $\ww$ and demanding stationarity, we have
\be
\sum_m {y^m\ww\cdot\xx^m\int\lambda^m(u) du}=0
\ee
Now we rewrite the lagrangian as
\begin{align}
\mathcal{L}\left(\ww,\xi^i(u),\lambda_i(u),\delta_i(u)\right)=&\sum_m {1\over\sqrt{2\pi\beta}}\int e^{-{u^2\over 2\beta}}\xi^m(u) du -\sum_m{\int{\lambda^m(u) \xi^m(u)} du} \nonumber \\
+&\sum_m{\int{\lambda^m(u)} du} +\sum_m{\int{u\lambda^m(u)} du}  \nonumber \\ - &\sum_m {\int\delta^m(u)\xi^m(u) du}= \\
&\sum_m {1\over\sqrt{2\pi\beta}}\int e^{-{u^2\over 2\beta}}\xi^m(u) du -\sum_m{\int{\lambda^m(u) \xi^m(u)} du} \nonumber \\
+&\sum_m{\int{\lambda^m(u)} du} +\sum_m{\int{u\lambda^m(u)} du}  \nonumber \\ - &\sum_m {\int{\left({1\over\sqrt{2\pi\beta}}e^{-{u^2\over 2\beta}}-\lambda^m(u)\right)\xi^m(u)} du} =\\
&\sum_m{\int{\lambda^m(u)} du} +\sum_m{\int{u\lambda^m(u)} du}
\end{align}
Applying a common trick to eliminate $\delta^i(u)$ we end up with
\be
\max_{\lambda^1(u),\lambda^2(u),...,\lambda^N(u)}\sum_m{\int{(u+1)\lambda^m(u)} du}
\ee
\be
\text{s.t. } \forall i\forall u\quad 0\leq\lambda^i(u)\leq  {1\over\sqrt{2\pi\beta}}e^{-{u^2\over 2\beta}}
\ee
Amir, is the problem you have found in the coffee shop present here too? if so, please explain it again. anyway, the problem that I have worked on here is undoubtly convex, so the problem must be something else.


==> dual.tex <==
\section{Deriving the dual}

As previously discussed, $L$ is a convex monotone decreasing function. Thus, inroducing an auxilliary $\xi^m=y^m\ww^T\xx^m$ and requiring that the inequallity $\xi^m\le y^m\ww^T\xx^m$ would not change the optimal value of the objective. The lagrangian of the problem at hand is thus
\begin{align}
\mathcal{L}(\ww,\xi,\lambda,\mu)=&\sum_m\left[(1-\xi^m){erf}_1\left({1-\xi^m\over{\sigma\|w\|}}\right)+{\sigma\|w\|\over{\sqrt{2\pi}}}
\exp\left({-{(1-\xi^m)^2\over{2\sigma^2\|w\|^2}}}\right)\right] \nonumber\\
+&\sum_m{\lambda_m\left(\xi^m-y^m\ww^T\xx^m\right)}+\mu(\|w\|-1)
\end{align}

Notice that instead of $\xi$ we could have use the variable $\mu^m=1-y^m\ww^T\xx^m$. In that case The probelm will take the following form:
\begin{align}
\mathcal{L}(\ww,\mu,\lambda)=&\sum_m\left[\mu^m{erf}_1\left({\mu^m\over{\sigma\|\ww\|}}\right)+{\sigma\|\ww\|\over{\sqrt{2\pi}}}
\exp\left({-{{\mu^m}^2\over{2\sigma^2\|w\|^2}}}\right)\right] \nonumber\\
-&\sum_m{\lambda_m\left(1-y^m\ww^T\xx^m-\mu^m\right)}
\end{align}

In that case the derviatives w.r.t the primals are:

\be
{\partial{\mathcal{L}}\over{\partial{\ww}}}=
{\ww\sigma\over{\|\ww\|\sqrt{2\pi}}}\sum_m{\exp{\left(-{{\mu^m}^2\over{2\sigma^2\|\ww\|^2}}\right)}}
+\sum_m{\lambda_m y^m\xx^m}
\ee
\be
{\partial{\mathcal{L}}\over{\partial{\mu^m}}}=
erf_1{\mu^m\over{\sigma\|\ww\|}}+\lambda_m
\ee
Denote $inverf$ the inverse function of $erf$ and $A(x)=\exp{-{inverf(-x)^2\over{2}}}$. Working around this eqs, we get that

\be
\mathcal{L}={\sum_{m,l}{y^my^l\lambda_m\lambda_l\left<\xx^m,\xx^l\right>}\over{{\sigma\over{\sqrt{2\pi}\|\ww\|}}\sum_m{A(\lambda_m)}}}
+{\sigma\over{\sqrt{2\pi}}}\sum_m{A(\lambda_m)}-\sum_m{\lambda_m}
\ee

s.t. $\lambda_m\ge 0$.


==> relWork.tex <==
\section{Related Work}


==> robgaus_bound.tex <==
\thm A simple bound on the norm of the optimal classifier\ethm
\prf
The loss function we are dealing with is
 \begin{align}
L_{\sigma^2}(\xx^m,y^m;\ww)=\left(1-y^m\ww^T\xx^m\right) \erf\left({{1-y^m\ww^T\xx^m}\over{\sigma\|\ww\|}}\right)\nonumber\\
+{\sigma\|\ww\|\over\sqrt{2\pi}}\exp{\left(-{\left(1-y^m\ww^T\xx^m\right)^2\over {2\sigma^2\|\ww\|^2}}\right)}
\end{align}
As you have suggested, this can be reformulated as
\be
L_{\sigma^2}(\xx^m,y^m;\ww) = \sigma\|\ww\|f\left(\frac{1-y^m\ww\cdot\xx^m}{\sigma\|\ww\|}\right)
\ee
where \be
f(z) = z\erf(z)+{1\over{\sqrt{2\pi}}}e^{-{z^2\over 2}}
\ee
The learning task can thus be expressed as
\begin{align}
\min_{\ww\in\mathbb{R}^d}{\sum_m{L_{\sigma^2}(\xx^m,y^m;\ww)}}
\end{align}
Denote by $\ww^*$ the optimal solution. By definition, for all $\uu\in\mathbb{R}^d$ it holds that
$$\sum_m{L_{\sigma^2}(\xx^m,y^m;\ww^*)}\leq\sum_m{L_{\sigma^2}(\xx^m,y^m;\uu)}$$
As discussed, plugging the zero vector as parameter into the loss functions yields a unit constant loss function. We thus have
$$\sum_m{L_{\sigma^2}(\xx^m,y^m;\ww^*)}\leq M$$
where $M$ is the size of the training set. Denote $m^*=\arg\min_{m=1..M}{L_{\sigma^2}(\xx^m,y^m;\ww^*)}$.
We conclude that
$$M\cdot L_{\sigma^2}(\xx^{m^*},y^{m^*};\ww^*)\leq M$$
Further denote $\tilde{z}=1-y^{m^*}{\ww^*}^T\xx^{m^*}$. It holds that $\tilde{z}\geq 0$. sketch of proof: otherwise just rescale $\ww$ or in the case of biased classifier $(\ww,b)$ so that the minimum is $\tilde{z}=0$. This is not rigorous but I think it is correct. what do you say? \newline
Now, as discussed, $f$ is convex in its argument, whence $f(x)\geq f(x_0)+f'(x_0)(x-x_0)$. We choose $x_0=0$ and get the inequality
\begin{align}
f\left({{1-y^m{\ww^*}^T\xx^m}\over{\sigma\|\ww^*\|}}\right)&\geq f(0)+f'(0){{1-y^m{\ww^*}^T\xx^m}\over{\sigma\|\ww^*\|}}=\nonumber\\
&={1\over{\sqrt{2\pi}}}+\half{{(1-y^m{\ww^*}^T\xx^m)}\over{\sigma\|\ww^*\|}}
\end{align}

Plugging this into eq. we get that
$$\sigma\|\ww^*\|\left({1\over{\sqrt{2\pi}}}+\half{{\tilde{z}}\over{\sigma\|\ww^*\|}}\right)\leq 1$$
Using the positivity of $\tilde{z}$ we conclude that
$$\|\ww^*\|\leq {\sqrt{2\pi}\over\sigma}$$

\eprf

